Generalized non-exponential Gaussian splatting

In this work we generalize 3D Gaussian splatting (3DGS) to a wider family of physically-based alpha-blending operators. 3DGS has become the standard de-facto for radiance field rendering and reconstruction, given its flexibility and efficiency. At its core, it is based on alpha-blending sorted semitransparent primitives, which in the limit converges to the classic radiative transfer function with exponential transmittance. Inspired by recent research on non-exponential radiative transfer, we generalize the image formation model of 3DGS to non-exponential regimes. Based on this generalization, we use a quadratic transmittance to define sub-linear, linear, and super-linear versions of 3DGS, which exhibit faster-than-exponential decay. We demonstrate that these new non-exponential variants achieve similar quality than the original 3DGS but significantly reduce the number of overdraws, which result on speed-ups of up to $4\times$ in complex real-world captures, on a ray-tracing-based renderer.

==> srcXX_other.tex <==


% -------------------------------------------------------------------

\section{Adjoint: Exponential transmittance}

Radiance along is computed as a weighted sum, where the weight as given by the product of the
transmittance of the primitives encountered so far:
\begin{align*}
    L_0 = \sum_{i=0}^N \left( E_i \alpha_i \cdot \prod_{j=0}^{i-1} (1 - \alpha_j) \right)
\end{align*}

Which can also be written in a recursive form:
\begin{align*}
    L_i = E_i \cdot \alpha_i  + (1 - \alpha_i) \cdot L_{i+1}
\end{align*}

In path replay, we compute the full radiance along the path in a first pass, given us $L_0$. In order to compute the other radiance terms, we note that
\begin{align*}
    L_{i+1} = \frac{L_{i} - E_i \cdot \alpha_i}{(1 - \alpha_i)}
\end{align*}

Let's look as what happens when differentiating these terms:
\begin{align*}
    \delta L_i = \delta (E_i \cdot \alpha_i) - \delta \alpha_i \cdot L_{i+1} + (1 - \alpha_i) \cdot \delta L_{i+1}
\end{align*}

% -------------------------------------------------------------------
\section{An approximated linear transmittance}
Unfortunately, the linear transmittance includes a clamping operator that makes differentiation challenging. Given the generality of our framework, we test an approximately linear transmittance operator, based on the softplus function, following
\begin{equation}
    T_{\text{soft}}(\tau) = \frac{1}{\log\left(1 +\exp(\kappa)\right)}\log\left(1 +\exp(\kappa-\kappa\tau)\right) \approx \frac{1}{\kappa}\log\left(1 +\exp(\kappa-\kappa\tau)\right), 
\end{equation}
with $\kappa$ an arbitrarily high constant. This transmittance function follows all requirements for transmittance functions, including $T(0)= 1$ and having zero or negative gradient in the whole domain. Following our recipe above, we can compute the image formation model for Gaussian splats using this transmittance function by computing the path-length distribution $p(t)$ as
\begin{equation}
    p_\text{soft}(\tau) = \frac{\kappa\,\exp(\kappa)\,\sigma_i}{\log\left(1+\exp(\kappa)\right)\,(\exp(\kappa\tau) + \exp(\kappa))} \approx \frac{\exp(\kappa)\,\sigma_i}{\exp(\kappa\tau) + \exp(\kappa)}
\end{equation}
which leads to the following radiance estimate
\begin{equation}
    L_0 = \sum_{i=0}^N \left( E_i \, \frac{\exp(\kappa)\,\alpha_i}{\exp(\sum_{j<i}\alpha_j) + \exp(\kappa)} \right).
\end{equation}
%
%and a discrete transmittance with the form:
%\begin{equation}
%    T_{\text{soft},i} = \prod_{j<i} (1 - \frac{\exp(\kappa)\,\alpha_i \left(\exp(\sum_{j<i}\alpha_j) + \exp(\kappa)\right)^{-1}}{\log\left(1 +\exp(\kappa-\sum_{j<i}\alpha_j)\right)})
%\end{equation}



% -------------------------------------------------------------------





% -------------------------------------------------------------------

\section{Adjoint: Linear transmittance (OLD!)}

\todo{Should we account for the $\max()$ here?}

\seb{I believe we can ignore the max operator as in practice we are not iterating over all primitives (e.g. in the sum) but stopping when this max operator saturates. So the $N$ here is adaptive, and guaranties that the sum will never go beyond $1$.}

In the case of linear transmittance, the alpha blender should be summed instead of multiplied:
\begin{align*}
    L_0 &= \sum_{i=0}^N \left( E_i \cdot \alpha_i \cdot (1 - \sum_{j=0}^{i-1} \alpha_j) \right) \\
        &= \sum_{i=0}^N E_i \cdot \alpha_i - \sum_{i=0}^N \left( E_i \cdot \alpha_i \cdot \sum_{j=0}^{i-1} \alpha_j \right)
\end{align*}

Looking at the second sum, with can expand it as:
\begin{align*}
    \sum_{i=0}^N \left( E_i \cdot \alpha_i \cdot \sum_{j=0}^{i-1} \alpha_j \right)
        &= 0 \cdot E_0 \cdot \alpha_0 + \alpha_0 \cdot E_1 \cdot \alpha_1 + (\alpha_0 + \alpha_1) \cdot E_2 \cdot \alpha_2 + ... \\
        &= \alpha_0 \cdot (E_1 \cdot \alpha_1 + E_2 \cdot \alpha_2 + ...) + \alpha_1 \cdot (E_2 \cdot \alpha_2 + E_3 \cdot \alpha_3 + ...) \\
        &= \sum_{i=0}^N \left( \alpha_i \cdot \sum_{j=i+1}^{N} E_j \cdot \alpha_j \right)
\end{align*}

Which can be written recursively as
\begin{align*}
    L_i &= E_i \cdot \alpha_i - E_i \cdot \alpha_i \cdot \sum_{j=0}^{i-1} \alpha_j + L_{i+1} \\
     &= E_i \cdot \alpha_i - \alpha_i \cdot \sum_{j=i+1}^{N} E_j \cdot \alpha_j + L_{i+1} \\
\end{align*}


Now taking the derivative and using the produce rule, we get:
\begin{align*}
    \delta L_0
        &= \sum_{i=0}^N \delta (E_i \cdot \alpha_i) - \sum_{i=0}^N \left( \delta (E_i \cdot \alpha_i) \cdot \sum_{j=0}^{i-1} \alpha_j \right) - \sum_{i=0}^N \left( E_i \cdot \alpha_i \cdot \sum_{j=0}^{i-1} \delta \alpha_j \right) \\
        &= \sum_{i=0}^N \delta (E_i \cdot \alpha_i) - \sum_{i=0}^N \left( \delta (E_i \cdot \alpha_i) \cdot \sum_{j=0}^{i-1} \alpha_j \right) - \sum_{i=0}^N \left( \delta \alpha_i \cdot \sum_{j=i+1}^{N} E_j \cdot \alpha_) \right) \\
        &= \sum_{i=0}^N \left( \delta (E_i \cdot \alpha_i) - \delta (E_i \cdot \alpha_i) \cdot \sum_{j=0}^{i-1} \alpha_j - \delta \alpha_i \cdot \sum_{j=i+1}^{N} E_j \cdot \alpha_j \right) \\
        &= \sum_{i=0}^N \left( \delta (E_i \cdot \alpha_i) - \delta (E_i \cdot \alpha_i) \cdot \Phi_i - \delta \alpha_i \cdot \Theta_i \right)
\end{align*}

With

\begin{itemize}
    \item $\Phi_i = \sum_{j=0}^{i-1} \alpha_j \rightarrow$ this term can be trivially computed in the backward pass, simply summing the $\alpha_i$ of the previous bounces.
    \item $\Theta_i = \sum_{j=i+1}^{N} E_j \cdot \alpha_j \rightarrow$ this term should be pre-computed as $\Theta_0 = \sum_{j=1}^{N} E_j \cdot \alpha_j$ and we can then recursively compute $\Theta_i = \Theta_{i-1} - E_i \cdot \alpha_i$
\end{itemize}

With this, we can come up with a recursive formula to compute the derivatives:
\begin{align*}
    \delta L_i = \delta E_i - \delta E_i \cdot \Phi_i - \delta \alpha_i \cdot \Theta_i + \delta L_{i+1}
\end{align*}

\begin{align*}
\Phi_i =
\begin{cases}
  0
  & i = 0 \\
  \Phi_{i-1} + \alpha_i
  & i > 0 \\
\end{cases}
\end{align*}

\begin{align*}
\Theta_i =
\begin{cases}
  \sum_{j=1}^{N} E_j \cdot \alpha_j
  & i = 0 \\
  \Theta_{i-1} - E_i \cdot \alpha_i
  & i > 0 \\
\end{cases}
\end{align*}

\subsection{Adjoint: Mixed linear-exponential transmittance function (OLD!)}

\todo{Need to derive the math for the mixed transmittance function}

\paragraph{Option 1: single global mixture value}

\begin{align*}
    T(t) = g \cdot (1-\int \alpha(x_s) ds) + (1-g) \exp(-\int \alpha(x_s) ds)
\end{align*}

\begin{align*}
    \rho_i = g \cdot \max(1-\sum_{j<i}(\alpha_j), 0) + (1-g) \cdot \prod_{j<i}(1-\alpha_j)
\end{align*}

\paragraph{Option 2: an individual g per primitive}

\begin{align*}
    T(t) = 1-\int \alpha(x_s) g(x_s) ds + \exp(-\int \alpha(x_s) (1-g(x_s)) ds)
\end{align*}

\begin{align*}
    \rho_i = \max(1-\sum_{j<i}(\alpha_j \cdot  \gamma_j), 0) + \prod_{j<i}(1-\alpha_j \cdot  (1-\gamma_j))
\end{align*}

We want to be able to optimize $g$ per primitive, hence we will go with the second option.

So we get (ignoring the $\max()$ operator for now):

\begin{align*}
    L_0 &= \sum_{i=0}^N \left( E_i \cdot \alpha_i \cdot \left( (1 - \sum_{j=0}^{i-1}(\alpha_j \cdot  \gamma_j)) + \prod_{j=0}^{i-1}(1-\alpha_j \cdot  (1-\gamma_j)) \right) \right) \\
        &= \sum_{i=0}^N \left( E_i \cdot \alpha_i \cdot (1 - \sum_{j=0}^{i-1}(\alpha_j \cdot  \gamma_j)) \right) + \sum_{i=0}^N \left( E_i \cdot \alpha_i \cdot \prod_{j=0}^{i-1}(1-\alpha_j \cdot (1-\gamma_j)) \right) \\
         &= L_0^{\text{lin}} + L_0^{\text{exp}}
\end{align*}

We can re-use the math above for the two terms recursively:

\begin{align*}
    L_i^{lin} &= E_i \cdot \alpha_i - E_i \cdot \alpha_i \cdot \sum_{j=0}^{i-1} (\alpha_j \cdot \gamma_j) + L_{i+1}^{lin} \\
    L_i^{exp} &= E_i \cdot \alpha_i + (1-\alpha_i \cdot (1-\gamma_i)) \cdot L^{exp}_{i+1}
\end{align*}

So we have 


\begin{align*}
    L_i &= L_{i}^{lin} + L_i^{exp} \\
        &= E_i \cdot \alpha_i - E_i \cdot \alpha_i \cdot \sum_{j=0}^{i-1} (\alpha_j \cdot \gamma_j) + E_i \cdot \alpha_i + (1-\alpha_i \cdot (1-\gamma_i)) \cdot L^{exp}_{i+1} + L_{i+1}^{lin} \\
        &= 2E_i \cdot \alpha_i - E_i \cdot \alpha_i \cdot \sum_{j=0}^{i-1} (\alpha_j \cdot \gamma_j) - \alpha_i \cdot (1-\gamma_i) \cdot L^{exp}_{i+1} + L_{i+1}
\end{align*}

And then take the derivatives:

\begin{align*}
    \delta L_i^{\text{lin}} &= \delta (E_i \cdot \alpha_i)  - \delta (E_i \cdot \alpha_i)  \cdot \Phi_i - \delta (\alpha_i \cdot \gamma_i) \cdot \Theta_i + \delta L_{i+1}^{\text{lin}} 
\end{align*}

\begin{align*}
\Phi_i =
\begin{cases}
  0
  & i = 0 \\
  \Phi_{i-1} + \alpha_i \cdot  \gamma_i
  & i > 0 \\
\end{cases}
\end{align*}

\begin{align*}
\Theta_i =
\begin{cases}
  \sum_{j=1}^{N} E_j \cdot \alpha_j
  & i = 0 \\
  \Theta_{i-1} - E_i \cdot \alpha_i
  & i > 0 \\
\end{cases}
\end{align*}
    
\begin{align*}
    \delta L_i^{\text{exp}} &= \delta (E_i \cdot \alpha_i) + \delta (1-\alpha_i \cdot (1-\gamma_i)) \cdot L_{i+1}^{\text{exp}} + (1-\alpha_i \cdot (1-\gamma_i)) \cdot \delta L_{i+1}^{\text{exp}} 
\end{align*}

